Test-Time Mixup Augmentation for Data and Class-Specific Uncertainty Estimation in Deep Learning Image Classification

Uncertainty estimation of trained deep learning networks is valuable for optimizing learning efficiency and evaluating the reliability of network predictions. In this paper, we propose a method for estimating uncertainty in deep learning image classification using test-time mixup augmentation (TTMA). To improve the ability to distinguish correct and incorrect predictions in existing aleatoric uncertainty, we introduce TTMA data uncertainty (TTMA-DU) by applying mixup augmentation to test data and measuring the entropy of the predicted label histogram. In addition to TTMA-DU, we propose TTMA class-specific uncertainty (TTMA-CSU), which captures aleatoric uncertainty specific to individual classes and provides insight into class confusion and class similarity within the trained network. We validate our proposed methods on the ISIC-18 skin lesion diagnosis dataset and the CIFAR-100 real-world image classification dataset. Our experiments show that (1) TTMA-DU more effectively differentiates correct and incorrect predictions compared to existing uncertainty measures due to mixup perturbation, and (2) TTMA-CSU provides information on class confusion and class similarity for both datasets.

==> SEC/2_Related.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%% Subsection 2.2. Mixup Augmentation 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Mixup augmentation}
\label{sec:mixup}

% Mixup은 이러이러한 것인데 이러이러한 우수성이 있어서 이러이러한 분야에 활용되어 우수한 결과를 보였다.
% Mixup is one of the recently proposed data augmentation techniques and is referred to as the earlier model of consistency regularization methods called \textit{mixed sample data augmentation}~\citep{Zhang2018}. The basic idea of mixup is to create synthetic training examples by linearly interpolating between pairs of training examples and their labels. The interpolation is performed using a convex combination, where the weight of each example is determined by a mixing coefficient alpha drawn from a beta distribution. Mixup has been shown to improve the generalization performance of deep neural networks on a variety of tasks, including image recognition~\citep{Yun2019,resizemix,Kim2020,saliencymix,supermix}, semantic segmentation~\citep{msdaseg1,msdaseg2,msdaseg3,msdaseg4,msdaseg5}, natural language processing~\citep{msdanlp1,msdanlp3,msdanlp3,msdanlp4,msdanlp5,msdanlp6}, video processing~\citep{msdavideo1,msdavideo2,msdavideo3,msdavideo4}, and medical image analysis~\citep{msdamed1,msdamed2,msdamed3,msdamed4,msdamed5,Verma2018,msdamed7}.
Mixup is a recently proposed data augmentation technique that creates synthetic training examples by interpolating between pairs of examples and their labels using a convex combination. 
The weight of each example is determined by a mixing coefficient $\alpha$ which is drawn from a beta distribution. 
This technique, which was first introduced by Zhang~\textit{et al.}, is considered a variation of consistency regularization methods, specifically mixed sample data augmentation~\citep{Zhang2018}. 
Mixup has been shown to improve the generalization performance of deep neural networks on a variety of tasks, including image recognition~\citep{Yun2019,resizemix,Kim2020,saliencymix,supermix}, semantic segmentation~\citep{msdaseg1,msdaseg2,msdaseg3,msdaseg4,msdaseg5}, natural language processing~\citep{msdanlp1,msdanlp3,msdanlp3,msdanlp4,msdanlp5,msdanlp6}, video processing~\citep{msdavideo1,msdavideo2,msdavideo3,msdavideo4}, and medical image analysis~\citep{msdamed1,msdamed2,msdamed3,msdamed4,msdamed5,Verma2018,msdamed7}. 
The simplicity and effectiveness of Mixup make it a valuable tool for deep learning practitioners to consider when working on a wide range of applications.


% Mixup은 최근 이러이러한 방법으로도 확장되고 있다.
Since the original proposal of mixup, there have been several related works that have extended the idea in various ways.
Verma~\textit{et al.} suggested a variant of mixup called Manifold Mixup, which uses geodesic interpolation on the hidden representations of the data instead of interpolating between the data and its labels~\citep{Verma2018}.
Yun~\textit{et al.} proposed CutMix, which creates synthetic training examples by combining sub-regions of multiple images and their labels~\citep{Yun2019}.
CutMix has been shown to be particularly effective for object detection tasks, where it can improve the localization performance of the model.
Kim~\textit{et al.} suggested PuzzleMix, which creates synthetic training examples by jigsaw shuffling and linearly interpolating between pairs of images~\citep{Kim2020}.
Hendrycks~\textit{et al.} proposed AugMix which creates synthetic training examples by applying a series of random image transformations to a single image, rather than interpolating between multiple images as in mixup~\citep{Hendrycks2020}.
AugMix has been shown to improve the robustness of models to various types of image perturbations, such as noise, blur, and color distortion.
Liu~\textit{et al.} suggested AutoMix that uses reinforcement learning to learn an optimal mixing strategy, by searching over different data augmentation techniques and interpolation coefficients~\citep{Liu2021}.

% Mixup이 어떤 역할을 하는지에 대해서는 이러이러한 연구가 선행되어 있다.
Various attempts have also been made to explain the effect and behavior of mixup.
Thulasidasan~\textit{et al.} found that mixup training can improve the calibration of deep neural networks, which means that the predicted probabilities of the model are more closely aligned with the true underlying probabilities of the data~\citep{Thulasidasan2019}.
Zhang~\textit{et al.} further showed that the effect of the mixup on calibration is highly dependent on the specific characteristics of the data and the model~\citep{Zhang2021}.
Wen~\textit{et al.} observed that combining ensembles and data augmentation can lead to significant degradation in the calibration of machine learning models~\citep{Wen2021}.
They also provided a theoretical analysis of the reasons for this effect and suggested that it may be due to the increased complexity of the model and the increased variance in predictions.
Zhang~\textit{et al.} also provided the theoretical analysis on how the mixup improves generalization and robustness to the adversarial attacks by proving that the mixup is approximately a regularized loss minimization.

% There are two unique characteristics of mixup augmentation.
% First, the mixup is a much more aggressive perturbation than the affine transform since the mixup changes the object appearance and texture of a \textit{target} image through a linear combination with another \textit{partner} image.
% Second, the mixup has a variable for selection of mixup partners; we can perform mixup on a target image with the partners uniformly sampled from all classes, or we can sample the mixup partners from a specific class to observe between-class relationship.
